FLoBC: A Decentralized Blockchain-Based Federated Learning Framework

The rapid expansion of data worldwide invites the need for more distributed solutions in order to apply machine learning on a much wider scale. The resultant distributed learning systems can have various degrees of centralization. In this work, we demonstrate our solution FLoBC for building a generic decentralized federated learning system using blockchain technology, accommodating any machine learning model that is compatible with gradient descent optimization. We present our system design comprising the two decentralized actors: trainer and validator, alongside our methodology for ensuring reliable and efficient operation of said system. Finally, we utilize FLoBC as an experimental sandbox to compare and contrast the effects of trainer-to-validator ratio, reward-penalty policy, and model synchronization schemes on the overall system performance, ultimately showing by example that a decentralized federated learning system is indeed a feasible alternative to more centralized architectures.

==> old_figs/main_elsevier.tex <==
% %% 
% %% Copyright 2019-2020 Elsevier Ltd
% %% 
% %% This file is part of the 'CAS Bundle'.
% %% --------------------------------------
% %% 
% %% It may be distributed under the conditions of the LaTeX Project Public
% %% License, either version 1.2 of this license or (at your option) any
% %% later version.  The latest version of this license is in
% %%    http://www.latex-project.org/lppl.txt
% %% and version 1.2 or later is part of all distributions of LaTeX
% %% version 1999/12/01 or later.
% %% 
% %% The list of all files belonging to the 'CAS Bundle' is
% %% given in the file `manifest.txt'.
% %% 
% %% Template article for cas-sc documentclass for 
% %% single column output.

% %\documentclass[a4paper,fleqn,longmktitle]{cas-sc}
% \documentclass[a4paper,fleqn]{cas-sc}

% %\usepackage[numbers]{natbib}
% %\usepackage[authoryear]{natbib}
% \usepackage[authoryear,longnamesfirst]{natbib}
% \usepackage[center]{caption}
% \usepackage{float}

% %%%Author macros
% \def\tsc#1{\csdef{#1}{\textsc{\lowercase{#1}}\xspace}}
% \tsc{WGM}
% \tsc{QE}
% \tsc{EP}
% \tsc{PMS}
% \tsc{BEC}
% \tsc{DE}
% %%%

% \begin{document}
% \let\WriteBookmarks\relax
% \def\floatpagepagefraction{1}
% \def\textpagefraction{.001}
% \shorttitle{Decentralized Learning Using Blockchain}
% \shortauthors{Ghanem et~al.}
% %\begin{frontmatter}

% %\title [mode = title]{A Study on Decentralized Blockchain-Based Federated Learning}               
% \title [mode = title]{FLoBC: A Decentralized Blockchain-Based Federated Learning Framework}  

% \address[1]{The American University in Cairo, New Cairo, Egypt\\Computer Science and Engineering Department}
% % \address[$\star$]{Computer Science and Engineering Department}


% \author{Mohamed Ghanem}
% \ead{oscar@aucegypt.edu}
% \author{Fadi Dawoud}
% \ead{fadiadel@aucegypt.edu}
% \author{Habiba Gamal}
% \ead{habibabassem@aucegypt.edu}
% \author{Eslam Soliman}
% \ead{eslam98@aucegypt.edu}
% \author{Hossam Sharara}
% \ead{hossam.sharara@aucegypt.edu}
% \author{Tamer El-Batt}
% \ead{tamer.elbatt@aucegypt.edu}

% \begin{abstract}
% %This paper presents FLoBC, a distributed, decentralized machine learning system that relies on the blockchain technology. This system, without data sharing, performs federated learning with training and validation distributed among the participating nodes. The system does not rely on particular model configurations and is generic for any stochastic gradient descent machine learning model. The focus of this paper is on the architecture, efficiency, and privacy of the distributed system. Experiments were conducted to determine the best performing ratio of trainers to validators, to monitor the performance of the model in the presence of malicious nodes and a reward/penalty feature, and to compare different synchronization schemes.
% The rapid expansion of data worldwide invites the need for more distributed solutions in order to apply machine learning on a much wider scale. The resultant distributed learning systems can have various degrees of centralization. In this work, we demonstrate our solution FLoBC for building a generic decentralized federated learning system using the blockchain technology, accommodating any GD-compatible\footnote{Compatible with gradient descent optimization} machine learning model. We present our system design comprising the two decentralized actors: \emph{trainer} and \emph{validator}, alongside our methodology for ensuring reliable and efficient operation of said system. Finally, we utilize FLoBC as an experimental sandbox to compare and contrast the effects of trainer-to-validator ratio, reward-penalty policy, and model synchronization schemes on the overall system performance, ultimately showing by example that a decentralized federated learning system is indeed a feasible alternative to more centralized architectures.
% \end{abstract}

% \begin{graphicalabstract}
% \centering
% \includegraphics[width=.8\textwidth]{figs/graphical_abstract.png}
% \end{graphicalabstract}

% \begin{highlights}
% \item Blockchain offers a viable solution for decentralized federated learning.
% \item Decentralized federated learning systems can perform comparably to centralized ones.
% \item Decentralized validation can handle both Byzantine trainers and validators.
% \end{highlights}

% \begin{keywords}
% Byzantine Fault-Tolerance \sep 
% Federated Learning \sep 
% Blockchain \sep 
% Decentralized Systems \sep 
% Distributed Machine Learning \sep 
% Privacy Preserving \sep 
% \end{keywords}


% \maketitle


% \input{introduction}
% \input{bg_related_work}
% \input{methodology}
% \input{architecture}
% \input{experiments}
% \input{conclusion}
% \input{future_work}




% %\appendix
% %\section{My Appendix}



% \bibliographystyle{plain}

% %% Loading bibliography style file
% %\bibliographystyle{model6-num-names}


% % Loading bibliography database
% \bibliography{ref}


% \end{document}


